EvoST: Adapting Traffic Forecasters to Evolving Sensor Graphs

Web-based navigation and traffic information services depend on accurate forecasts as sensor networks evolve. On checkpoints reused years later, updating only shared weights or adding a low-rank node prompt leaves substantial degradation, whereas, in the evaluated architectures, refreshing node identities recovers most of it while the shared spatio-temporal weights are reused. We propose EvoST, a framework that maintains traffic forecasters by refreshing node identities while keeping shared weights fixed. EvoST updates existing identities using recently released labels and initializes new sensors with identities borrowed from behaviorally similar established sensors. Once enough delayed labels arrive, it jointly refits all identities, and a per-sensor recursive least-squares calibrator corrects forecasts as labels become available. Across twelve PeMS region-year settings, identity refresh reduces the relative one-hour MAE gap between five-year-old STAEFormer checkpoints and target-year models from 17.7% to 2.5%, with all forecasters calibrated, and its MAE is 0.7% above that of full-parameter fine-tuning on the same data. In Graph WaveNet, identity refresh recovers 88% of the five-year MAE gap to calibrated target-year models. Similar recovery holds for STAEFormer checkpoints up to fifteen years old, while refreshing STID recovers 67% of its five-year gap. On an annual benchmark covering nine EvoXXLTraffic districts and Transport for NSW, EvoST has the lowest average MAE, RMSE, and MAPE among the reported non-foundation methods on all ten networks, and calibration accounts for most of its Avg-MAE reduction from the matched frozen checkpoints. Code and the extended version: https://github.com/lixus7/EvoST

==> table/evost_arrival.tex <==
\begin{table}[t]
\centering
\caption{Strict arrival, test portion after the refit event. New and All use the calibrated target-year reference. Established uses the same mature model without new sensors as its reference. All entries are relative H12 MAE.}
\label{tab:arrival}
\begin{tabular}{lrrr}
\toprule
Strategy & New & All & Established \\
\midrule
Borrow and keep & 1.115 & 1.052 & 1.008 \\
Refit new identities & 1.038 & 1.035 & 1.008 \\
Refit all (EvoST) & 1.036 & 1.032 & 1.003 \\
\bottomrule
\end{tabular}
\end{table}


==> table/evost_cost.tex <==
\begin{table}[htbp]
\centering
\caption{Median fitting costs in the primary STAEFormer maintenance experiment (H100 runs). Search time includes three learning-rate candidates. These are fitting costs, excluding calibration.}
\label{tab:cost}
\begin{tabular}{lrrrr}
\toprule
Updated group & Values & s/epoch & Search (s) & GiB \\
\midrule
Identity refresh & 1.41M & 11.5 & 259 & 10.4 \\
Full fine-tuning & 2.01M & 14.0 & 327 & 11.4 \\
Shared weights & 0.60M & 13.7 & 334 & 11.6 \\
Output head & 0.02M & 4.8 & 180 & 4.5 \\
\bottomrule
\end{tabular}
\end{table}


==> table/evost_horizons.tex <==
\begin{table*}[t]
\centering
\caption{Additional primary test metrics, normalized to the calibrated target-year reference. H3, H6, and H12 aggregate errors over steps 1--3, 1--6, and 1--12 (15, 30, and 60 minutes). Avg. MAE averages the twelve cumulative-horizon MAEs.}
\label{tab:horizons}
\begin{tabular}{lrrrrr}
\toprule
Maintenance & H3 MAE & H6 MAE & H12 MAE & H12 RMSE & Avg. MAE \\
\midrule
Old checkpoint & 1.075 & 1.111 & 1.177 & 1.154 & 1.117 \\
Output head & 1.064 & 1.093 & 1.148 & 1.129 & 1.098 \\
Shared weights & 1.033 & 1.049 & 1.078 & 1.069 & 1.051 \\
Added node prompt & 1.062 & 1.087 & 1.130 & 1.114 & 1.090 \\
Recent-data scratch & 1.061 & 1.084 & 1.123 & 1.117 & 1.086 \\
Identity refresh (EvoST) & 1.013 & 1.017 & 1.025 & 1.026 & 1.018 \\
Identities + prompt & 1.011 & 1.016 & 1.023 & 1.024 & 1.016 \\
All parameters & 1.007 & 1.011 & 1.018 & 1.021 & 1.012 \\
\bottomrule
\end{tabular}
\end{table*}


==> table/evost_main_absolute.tex <==
\begin{table*}[t]
\centering
\caption{Absolute test H12 MAE on the primary PeMS panel (mean of three seeds). All methods use calibration. Target-year is the separately trained current-year reference; scratch uses only the recent maintenance history. The old checkpoint is five years old; New denotes the fraction of nodes absent from it.}
\label{tab:absolute}
\begin{tabular}{lrrrrrrrrr}
\toprule
Region/year & Nodes & New & Target-year & Old & Shared & Prompt & Scratch & EvoST & Full FT \\
\midrule
PeMS03/2020 & 1213 & 8.1\% & 11.03 & 12.84 & 11.72 & 11.97 & 12.17 & 11.17 & 10.94 \\
PeMS03/2025 & 1859 & 45.1\% & 9.37 & 11.36 & 10.70 & 11.11 & 10.86 & 10.12 & 9.95 \\
PeMS06/2020 & 630 & 46.0\% & 10.20 & 13.03 & 11.20 & 12.01 & 11.54 & 10.60 & 10.51 \\
PeMS06/2025 & 746 & 24.4\% & 10.65 & 11.71 & 10.96 & 11.60 & 11.76 & 10.57 & 10.54 \\
PeMS08/2020 & 1991 & 24.8\% & 10.77 & 13.49 & 12.10 & 13.02 & 12.61 & 11.22 & 11.25 \\
PeMS08/2025 & 2074 & 12.0\% & 12.24 & 13.60 & 12.80 & 13.45 & 13.51 & 12.13 & 12.09 \\
PeMS10/2020 & 1152 & 32.3\% & 9.95 & 12.10 & 11.06 & 11.48 & 10.55 & 10.63 & 10.61 \\
PeMS10/2025 & 1396 & 21.3\% & 9.11 & 10.63 & 9.63 & 10.04 & 9.77 & 9.27 & 9.20 \\
PeMS11/2020 & 1488 & 12.3\% & 12.76 & 15.05 & 13.93 & 14.55 & 14.65 & 13.54 & 13.47 \\
PeMS11/2025 & 1440 & 5.4\% & 14.19 & 16.07 & 14.72 & 15.64 & 15.94 & 14.04 & 13.83 \\
PeMS12/2020 & 2420 & 11.4\% & 12.42 & 14.38 & 13.46 & 13.88 & 14.71 & 12.73 & 12.69 \\
PeMS12/2025 & 2587 & 10.0\% & 12.15 & 14.22 & 12.83 & 13.53 & 13.62 & 12.06 & 12.02 \\
\bottomrule
\end{tabular}
\end{table*}


==> table/evost_maintenance_summary.tex <==
\begin{table}[t]
\centering
\caption{Which parameters to maintain? Relative test H12 MAE against a target-year STAEFormer (1.000). All arms and the reference are calibrated. Geometric means over twelve settings; lower is better.}
\label{tab:maintenance}
\begin{tabular}{lrr}
\toprule
Maintained parameters & Ratio & 95\% interval \\
\midrule
Old checkpoint & 1.177 & [1.166, 1.187] \\
Output head & 1.148 & [1.138, 1.158] \\
Shared weights & 1.078 & [1.068, 1.089] \\
Added node prompt & 1.130 & [1.122, 1.140] \\
Recent-data scratch & 1.123 & [1.098, 1.141] \\
Identity refresh (EvoST) & 1.025 & [1.015, 1.037] \\
Identities + prompt & 1.023 & [1.014, 1.033] \\
All parameters & 1.018 & [1.010, 1.027] \\
\bottomrule
\end{tabular}
\end{table}


==> table/newsensor1.tex <==
\begin{table*}[t]
\centering
\caption{Newly-added-sensor forecast errors, part 1/2 (PEMS03, PEMS04, PEMS05, PEMS06, PEMS07; mean$\pm$std over seeds per dataset). Years where the graph did not grow are excluded. Baselines are grouped and ordered to match \Cref{tab:main_full}. \textbf{Bold}: best, \underline{underline}: second best.}
\label{tab:tsas_new_sensors_part1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccc|cccc|cccc|cccc|cc|cccc|c}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metric}} & \multirow{2}{*}{\textbf{Horizon}} & \multicolumn{4}{c|}{\textbf{Static STGNN Backbones}} & \multicolumn{4}{c|}{\textbf{Na\"ive Schemes}} & \multicolumn{4}{c|}{\textbf{Evolving-Graph Continual}} & \multicolumn{2}{c|}{\textbf{Retrieval / TTC}} & \multicolumn{4}{c|}{\textbf{Other Static Backbones}} & \multicolumn{1}{c}{\textbf{Ours}} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-11} \cmidrule(lr){12-15} \cmidrule(lr){16-17} \cmidrule(lr){18-21} \cmidrule(lr){22-22}
 &  &  & \textbf{DCRNN} & \textbf{ASTGNN} & \textbf{TGCN} & \textbf{GWN} & \textbf{Pretrain} & \textbf{Retrain} & \textbf{OL-NN} & \textbf{OL-AN} & \textbf{TrafStm} & \textbf{PECPM} & \textbf{STKEC} & \textbf{EAC} & \textbf{STRAP} & \textbf{ST-TTC} & \textbf{STID} & \textbf{STNorm} & \textbf{iTrans} & \textbf{DLinear} & \textbf{A2TTA} \\
\midrule
\multirow{12}{*}{\textbf{PEMS03}} & \multirow{4}{*}{MAE} & 3 & 19.05$_{\pm2.59}$ & 10.09$_{\pm0.14}$ & 18.49$_{\pm0.11}$ & 10.56$_{\pm0.19}$ & 25.21$_{\pm0.97}$ & \underline{9.35$_{\pm0.79}$} & 9.60$_{\pm0.08}$ & 9.40$_{\pm0.05}$ & 9.71$_{\pm0.15}$ & 10.48$_{\pm0.66}$ & 9.89$_{\pm0.21}$ & 10.67$_{\pm0.13}$ & 30.31$_{\pm1.06}$ & 9.72$_{\pm0.08}$ & 57.53$_{\pm5.42}$ & 12.10$_{\pm0.85}$ & 9.75$_{\pm0.07}$ & 10.21$_{\pm0.06}$ & \textbf{9.22$_{\pm0.06}$} \\
 &  & 6 & 19.27$_{\pm2.61}$ & 10.97$_{\pm0.13}$ & 18.86$_{\pm0.10}$ & 11.17$_{\pm0.14}$ & 25.53$_{\pm0.95}$ & \underline{9.98$_{\pm0.85}$} & 10.24$_{\pm0.11}$ & 10.06$_{\pm0.04}$ & 10.35$_{\pm0.17}$ & 11.08$_{\pm0.64}$ & 10.48$_{\pm0.16}$ & 11.61$_{\pm0.33}$ & 29.65$_{\pm0.72}$ & 10.38$_{\pm0.08}$ & 57.58$_{\pm5.49}$ & 12.95$_{\pm1.05}$ & 10.40$_{\pm0.07}$ & 11.12$_{\pm0.04}$ & \textbf{9.91$_{\pm0.07}$} \\
 &  & 12 & 20.27$_{\pm2.56}$ & 12.96$_{\pm0.13}$ & 19.93$_{\pm0.10}$ & 12.69$_{\pm0.20}$ & 26.46$_{\pm0.75}$ & \underline{11.32$_{\pm0.96}$} & 11.53$_{\pm0.19}$ & 11.40$_{\pm0.07}$ & 11.70$_{\pm0.26}$ & 12.38$_{\pm0.62}$ & 11.84$_{\pm0.13}$ & 13.66$_{\pm0.56}$ & 30.28$_{\pm2.71}$ & 11.78$_{\pm0.10}$ & 58.15$_{\pm5.39}$ & 14.94$_{\pm1.55}$ & 11.81$_{\pm0.07}$ & 13.21$_{\pm0.02}$ & \textbf{11.29$_{\pm0.10}$} \\
 &  & Avg & 19.45$_{\pm2.59}$ & 11.17$_{\pm0.13}$ & 19.01$_{\pm0.10}$ & 11.34$_{\pm0.15}$ & 25.66$_{\pm0.88}$ & \underline{10.10$_{\pm0.86}$} & 10.34$_{\pm0.12}$ & 10.17$_{\pm0.05}$ & 10.47$_{\pm0.19}$ & 11.20$_{\pm0.64}$ & 10.62$_{\pm0.17}$ & 11.81$_{\pm0.32}$ & 30.08$_{\pm0.54}$ & 10.50$_{\pm0.08}$ & 57.60$_{\pm5.44}$ & 13.17$_{\pm1.11}$ & 10.53$_{\pm0.07}$ & 11.33$_{\pm0.04}$ & \textbf{10.02$_{\pm0.07}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{RMSE} & 3 & 28.63$_{\pm2.49}$ & 16.95$_{\pm0.19}$ & 32.98$_{\pm0.34}$ & 17.53$_{\pm0.30}$ & 32.20$_{\pm1.00}$ & \underline{15.62$_{\pm1.34}$} & 16.13$_{\pm0.14}$ & 15.79$_{\pm0.11}$ & 16.13$_{\pm0.14}$ & 17.13$_{\pm0.83}$ & 16.40$_{\pm0.27}$ & 17.46$_{\pm0.23}$ & 46.63$_{\pm1.77}$ & 16.23$_{\pm0.09}$ & 98.72$_{\pm8.19}$ & 19.43$_{\pm1.03}$ & 16.24$_{\pm0.10}$ & 17.22$_{\pm0.04}$ & \textbf{15.43$_{\pm0.10}$} \\
 &  & 6 & 29.11$_{\pm2.49}$ & 18.76$_{\pm0.16}$ & 33.57$_{\pm0.33}$ & 18.76$_{\pm0.22}$ & 33.25$_{\pm0.95}$ & \underline{16.97$_{\pm1.46}$} & 17.46$_{\pm0.18}$ & 17.15$_{\pm0.12}$ & 17.49$_{\pm0.18}$ & 18.45$_{\pm0.79}$ & 17.71$_{\pm0.21}$ & 19.51$_{\pm0.60}$ & 46.23$_{\pm1.49}$ & 17.63$_{\pm0.11}$ & 98.87$_{\pm8.24}$ & 20.87$_{\pm1.24}$ & 17.54$_{\pm0.08}$ & 19.17$_{\pm0.02}$ & \textbf{16.82$_{\pm0.13}$} \\
 &  & 12 & 31.13$_{\pm2.38}$ & 22.67$_{\pm0.16}$ & 35.30$_{\pm0.30}$ & 21.76$_{\pm0.37}$ & 35.80$_{\pm0.74}$ & \underline{19.64$_{\pm1.67}$} & 19.99$_{\pm0.34}$ & 19.74$_{\pm0.17}$ & 20.16$_{\pm0.38}$ & 21.14$_{\pm0.78}$ & 20.49$_{\pm0.22}$ & 23.73$_{\pm1.09}$ & 49.16$_{\pm5.10}$ & 20.42$_{\pm0.13}$ & 99.61$_{\pm8.16}$ & 24.35$_{\pm1.90}$ & 20.25$_{\pm0.06}$ & 23.36$_{\pm0.01}$ & \textbf{19.50$_{\pm0.21}$} \\
 &  & Avg & 29.45$_{\pm2.47}$ & 19.11$_{\pm0.16}$ & 33.80$_{\pm0.33}$ & 19.10$_{\pm0.25}$ & 33.53$_{\pm0.86}$ & \underline{17.16$_{\pm1.47}$} & 17.62$_{\pm0.21}$ & 17.32$_{\pm0.12}$ & 17.68$_{\pm0.21}$ & 18.65$_{\pm0.80}$ & 17.94$_{\pm0.23}$ & 19.89$_{\pm0.58}$ & 47.18$_{\pm1.30}$ & 17.84$_{\pm0.11}$ & 98.90$_{\pm8.21}$ & 21.27$_{\pm1.33}$ & 17.76$_{\pm0.07}$ & 19.54$_{\pm0.02}$ & \textbf{17.00$_{\pm0.14}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{MAPE (\%)} & 3 & 74.40$_{\pm27.93}$ & \underline{28.76$_{\pm0.71}$} & 36.64$_{\pm1.86}$ & 32.27$_{\pm1.54}$ & 58.98$_{\pm4.12}$ & 30.11$_{\pm1.67}$ & 29.01$_{\pm0.74}$ & 29.40$_{\pm0.81}$ & 30.85$_{\pm1.23}$ & 33.49$_{\pm3.42}$ & 32.05$_{\pm0.95}$ & 34.80$_{\pm2.15}$ & 76.12$_{\pm17.29}$ & 31.05$_{\pm1.03}$ & 61.26$_{\pm2.88}$ & 55.66$_{\pm9.16}$ & 30.16$_{\pm0.41}$ & 29.48$_{\pm0.28}$ & \textbf{28.60$_{\pm0.41}$} \\
 &  & 6 & 74.81$_{\pm27.86}$ & 30.39$_{\pm0.70}$ & 37.04$_{\pm2.18}$ & 33.27$_{\pm1.67}$ & 57.79$_{\pm3.94}$ & 31.11$_{\pm1.65}$ & \underline{29.77$_{\pm0.89}$} & 30.08$_{\pm0.72}$ & 31.36$_{\pm1.46}$ & 34.15$_{\pm3.37}$ & 32.68$_{\pm1.07}$ & 36.55$_{\pm1.15}$ & 75.32$_{\pm18.52}$ & 32.08$_{\pm0.87}$ & 61.98$_{\pm3.04}$ & 57.86$_{\pm9.83}$ & 31.16$_{\pm0.40}$ & 31.56$_{\pm0.36}$ & \textbf{29.50$_{\pm0.38}$} \\
 &  & 12 & 76.89$_{\pm27.61}$ & 34.42$_{\pm0.76}$ & 40.28$_{\pm2.46}$ & 36.05$_{\pm1.89}$ & 57.02$_{\pm2.81}$ & 33.86$_{\pm1.90}$ & \underline{32.06$_{\pm1.90}$} & 32.36$_{\pm0.86}$ & 33.79$_{\pm2.64}$ & 36.24$_{\pm3.45}$ & 35.23$_{\pm1.34}$ & 41.76$_{\pm1.43}$ & 80.92$_{\pm21.82}$ & 34.91$_{\pm0.55}$ & 63.43$_{\pm2.64}$ & 63.56$_{\pm11.18}$ & 33.78$_{\pm0.18}$ & 37.14$_{\pm0.66}$ & \textbf{31.47$_{\pm0.33}$} \\
 &  & Avg & 75.13$_{\pm27.78}$ & 30.85$_{\pm0.73}$ & 37.72$_{\pm2.13}$ & 33.62$_{\pm1.69}$ & 58.10$_{\pm3.76}$ & 31.44$_{\pm1.70}$ & \underline{30.11$_{\pm1.02}$} & 30.41$_{\pm0.79}$ & 31.78$_{\pm1.67}$ & 34.40$_{\pm3.40}$ & 33.10$_{\pm1.10}$ & 37.22$_{\pm1.30}$ & 76.77$_{\pm18.54}$ & 32.42$_{\pm0.81}$ & 62.05$_{\pm2.87}$ & 58.56$_{\pm9.92}$ & 31.48$_{\pm0.33}$ & 32.27$_{\pm0.34}$ & \textbf{29.68$_{\pm0.38}$} \\
\midrule
\multirow{12}{*}{\textbf{PEMS04}} & \multirow{4}{*}{MAE} & 3 & 99.44$_{\pm10.40}$ & 16.47$_{\pm0.26}$ & 111.23$_{\pm1.42}$ & 18.43$_{\pm0.50}$ & 135.51$_{\pm6.16}$ & 16.12$_{\pm0.18}$ & 15.74$_{\pm0.28}$ & 15.70$_{\pm0.17}$ & \underline{15.66$_{\pm0.24}$} & 19.19$_{\pm4.22}$ & 16.80$_{\pm1.41}$ & 26.85$_{\pm8.49}$ & 91.01$_{\pm22.82}$ & 16.12$_{\pm0.18}$ & 96.85$_{\pm0.92}$ & 18.31$_{\pm0.91}$ & 16.05$_{\pm0.27}$ & 39.79$_{\pm2.85}$ & \textbf{14.75$_{\pm0.15}$} \\
 &  & 6 & 99.58$_{\pm10.36}$ & 18.04$_{\pm0.19}$ & 111.37$_{\pm1.39}$ & 19.25$_{\pm0.45}$ & 135.38$_{\pm5.92}$ & 17.31$_{\pm0.12}$ & \underline{16.81$_{\pm0.36}$} & 16.91$_{\pm0.22}$ & 16.85$_{\pm0.26}$ & 20.30$_{\pm4.08}$ & 17.79$_{\pm1.06}$ & 28.45$_{\pm8.00}$ & 89.69$_{\pm23.61}$ & 17.31$_{\pm0.12}$ & 97.07$_{\pm0.63}$ & 19.49$_{\pm0.77}$ & 17.21$_{\pm0.18}$ & 40.87$_{\pm2.80}$ & \textbf{16.05$_{\pm0.18}$} \\
 &  & 12 & 100.27$_{\pm10.23}$ & 21.56$_{\pm0.16}$ & 111.81$_{\pm1.35}$ & 22.00$_{\pm0.49}$ & 135.52$_{\pm5.96}$ & 19.97$_{\pm0.12}$ & \underline{19.07$_{\pm0.62}$} & 19.40$_{\pm0.26}$ & 19.35$_{\pm0.40}$ & 22.79$_{\pm3.93}$ & 20.43$_{\pm0.96}$ & 31.95$_{\pm6.55}$ & 87.04$_{\pm25.16}$ & 19.97$_{\pm0.12}$ & 97.45$_{\pm0.84}$ & 22.35$_{\pm0.53}$ & 19.82$_{\pm0.14}$ & 43.67$_{\pm2.68}$ & \textbf{18.70$_{\pm0.26}$} \\
 &  & Avg & 99.70$_{\pm10.33}$ & 18.39$_{\pm0.20}$ & 111.44$_{\pm1.39}$ & 19.67$_{\pm0.45}$ & 135.47$_{\pm5.97}$ & 17.58$_{\pm0.14}$ & \underline{17.01$_{\pm0.40}$} & 17.12$_{\pm0.21}$ & 17.07$_{\pm0.28}$ & 20.54$_{\pm4.09}$ & 18.12$_{\pm1.16}$ & 28.80$_{\pm7.75}$ & 89.42$_{\pm23.68}$ & 17.58$_{\pm0.14}$ & 97.22$_{\pm0.78}$ & 19.82$_{\pm0.75}$ & 17.47$_{\pm0.20}$ & 41.20$_{\pm2.81}$ & \textbf{16.27$_{\pm0.19}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{RMSE} & 3 & 120.58$_{\pm12.39}$ & 25.98$_{\pm0.28}$ & 169.79$_{\pm1.24}$ & 28.09$_{\pm0.48}$ & 168.45$_{\pm7.38}$ & 25.35$_{\pm0.21}$ & \underline{24.84$_{\pm0.19}$} & 24.85$_{\pm0.17}$ & 24.86$_{\pm0.25}$ & 29.72$_{\pm6.04}$ & 26.04$_{\pm1.39}$ & 38.57$_{\pm10.24}$ & 117.27$_{\pm25.98}$ & 25.35$_{\pm0.21}$ & 153.72$_{\pm0.83}$ & 28.28$_{\pm1.15}$ & 25.26$_{\pm0.27}$ & 51.59$_{\pm3.07}$ & \textbf{23.84$_{\pm0.15}$} \\
 &  & 6 & 120.77$_{\pm12.29}$ & 28.76$_{\pm0.21}$ & 169.75$_{\pm1.23}$ & 29.68$_{\pm0.52}$ & 168.62$_{\pm7.06}$ & 27.60$_{\pm0.15}$ & \underline{26.87$_{\pm0.37}$} & 27.05$_{\pm0.23}$ & 27.06$_{\pm0.28}$ & 31.75$_{\pm5.80}$ & 28.04$_{\pm1.01}$ & 41.20$_{\pm9.37}$ & 116.27$_{\pm26.59}$ & 27.60$_{\pm0.15}$ & 153.93$_{\pm0.82}$ & 30.19$_{\pm0.93}$ & 27.40$_{\pm0.17}$ & 54.05$_{\pm3.04}$ & \textbf{26.15$_{\pm0.20}$} \\
 &  & 12 & 121.72$_{\pm12.01}$ & 34.63$_{\pm0.21}$ & 169.73$_{\pm1.22}$ & 34.37$_{\pm0.76}$ & 169.82$_{\pm7.22}$ & 32.22$_{\pm0.20}$ & \underline{30.79$_{\pm0.88}$} & 31.28$_{\pm0.33}$ & 31.37$_{\pm0.51}$ & 36.04$_{\pm5.52}$ & 32.77$_{\pm1.11}$ & 46.82$_{\pm6.92}$ & 114.70$_{\pm28.14}$ & 32.22$_{\pm0.20}$ & 154.07$_{\pm1.02}$ & 34.75$_{\pm0.61}$ & 31.92$_{\pm0.19}$ & 59.49$_{\pm2.96}$ & \textbf{30.59$_{\pm0.35}$} \\
 &  & Avg & 120.93$_{\pm12.24}$ & 29.27$_{\pm0.23}$ & 169.76$_{\pm1.23}$ & 30.31$_{\pm0.52}$ & 168.89$_{\pm7.14}$ & 27.99$_{\pm0.18}$ & \underline{27.14$_{\pm0.44}$} & 27.35$_{\pm0.23}$ & 27.37$_{\pm0.32}$ & 32.12$_{\pm5.82}$ & 28.55$_{\pm1.17}$ & 41.75$_{\pm8.97}$ & 116.16$_{\pm26.70}$ & 27.99$_{\pm0.18}$ & 154.00$_{\pm0.71}$ & 30.69$_{\pm0.90}$ & 27.80$_{\pm0.21}$ & 54.57$_{\pm3.05}$ & \textbf{26.46$_{\pm0.22}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{MAPE (\%)} & 3 & 494.29$_{\pm62.84}$ & 21.49$_{\pm1.08}$ & 68.08$_{\pm4.13}$ & 23.23$_{\pm1.15}$ & 84.88$_{\pm2.60}$ & 21.86$_{\pm0.80}$ & 20.28$_{\pm1.01}$ & \underline{19.72$_{\pm0.41}$} & 21.33$_{\pm0.70}$ & 25.56$_{\pm5.26}$ & 24.61$_{\pm2.21}$ & 40.84$_{\pm17.97}$ & 70.46$_{\pm17.53}$ & 21.86$_{\pm0.80}$ & 43.91$_{\pm0.78}$ & 33.41$_{\pm3.65}$ & 22.32$_{\pm0.70}$ & 34.47$_{\pm3.29}$ & \textbf{19.35$_{\pm0.34}$} \\
 &  & 6 & 494.94$_{\pm62.44}$ & 23.03$_{\pm1.05}$ & 68.34$_{\pm4.18}$ & 23.92$_{\pm1.21}$ & 84.71$_{\pm2.71}$ & 22.96$_{\pm0.70}$ & 21.20$_{\pm1.27}$ & \underline{20.73$_{\pm0.37}$} & 22.33$_{\pm0.79}$ & 26.80$_{\pm5.30}$ & 25.14$_{\pm1.73}$ & 41.81$_{\pm16.49}$ & 69.02$_{\pm16.08}$ & 22.96$_{\pm0.70}$ & 44.29$_{\pm0.80}$ & 34.86$_{\pm3.53}$ & 23.20$_{\pm0.70}$ & 35.75$_{\pm3.11}$ & \textbf{20.22$_{\pm0.36}$} \\
 &  & 12 & 495.68$_{\pm62.28}$ & 27.12$_{\pm0.90}$ & 69.16$_{\pm4.27}$ & 26.23$_{\pm1.25}$ & 84.46$_{\pm2.82}$ & 25.99$_{\pm0.54}$ & 23.53$_{\pm1.97}$ & \underline{23.51$_{\pm0.42}$} & 25.29$_{\pm1.39}$ & 29.63$_{\pm5.00}$ & 27.74$_{\pm1.50}$ & 45.09$_{\pm15.05}$ & 67.94$_{\pm12.99}$ & 25.99$_{\pm0.54}$ & 45.53$_{\pm0.65}$ & 38.59$_{\pm3.56}$ & 25.55$_{\pm0.82}$ & 39.86$_{\pm2.93}$ & \textbf{22.20$_{\pm0.41}$} \\
 &  & Avg & 494.79$_{\pm62.38}$ & 23.53$_{\pm1.01}$ & 68.45$_{\pm4.21}$ & 24.28$_{\pm1.18}$ & 84.72$_{\pm2.69}$ & 23.35$_{\pm0.67}$ & 21.49$_{\pm1.36}$ & \underline{21.09$_{\pm0.34}$} & 22.75$_{\pm0.90}$ & 27.09$_{\pm5.17}$ & 25.55$_{\pm1.74}$ & 42.17$_{\pm16.61}$ & 69.19$_{\pm15.50}$ & 23.35$_{\pm0.67}$ & 44.51$_{\pm0.65}$ & 35.33$_{\pm3.57}$ & 23.52$_{\pm0.75}$ & 36.38$_{\pm3.11}$ & \textbf{20.43$_{\pm0.37}$} \\
\midrule
\multirow{12}{*}{\textbf{PEMS05}} & \multirow{4}{*}{MAE} & 3 & 8.41$_{\pm0.11}$ & 8.02$_{\pm0.05}$ & 8.24$_{\pm0.13}$ & 8.52$_{\pm0.14}$ & 20.46$_{\pm0.98}$ & 8.02$_{\pm0.09}$ & \underline{7.69$_{\pm0.06}$} & 7.74$_{\pm0.09}$ & 7.87$_{\pm0.18}$ & 8.17$_{\pm0.29}$ & 7.94$_{\pm0.16}$ & 11.48$_{\pm3.43}$ & 23.19$_{\pm5.81}$ & 8.02$_{\pm0.09}$ & 12.61$_{\pm4.42}$ & 9.10$_{\pm0.13}$ & 7.98$_{\pm0.17}$ & 8.13$_{\pm0.05}$ & \textbf{7.50$_{\pm0.08}$} \\
 &  & 6 & 8.64$_{\pm0.08}$ & 8.66$_{\pm0.05}$ & 8.58$_{\pm0.10}$ & 9.02$_{\pm0.15}$ & 20.77$_{\pm0.94}$ & 8.47$_{\pm0.08}$ & \underline{8.07$_{\pm0.06}$} & 8.18$_{\pm0.06}$ & 8.28$_{\pm0.18}$ & 8.62$_{\pm0.27}$ & 8.36$_{\pm0.13}$ & 11.92$_{\pm3.52}$ & 23.27$_{\pm5.85}$ & 8.47$_{\pm0.08}$ & 12.94$_{\pm4.39}$ & 9.46$_{\pm0.14}$ & 8.44$_{\pm0.14}$ & 8.81$_{\pm0.04}$ & \textbf{7.96$_{\pm0.06}$} \\
 &  & 12 & 9.39$_{\pm0.06}$ & 9.97$_{\pm0.07}$ & 9.43$_{\pm0.08}$ & 10.32$_{\pm0.17}$ & 21.62$_{\pm1.00}$ & 9.41$_{\pm0.10}$ & \underline{8.85$_{\pm0.09}$} & 9.04$_{\pm0.05}$ & 9.14$_{\pm0.21}$ & 9.57$_{\pm0.27}$ & 9.25$_{\pm0.13}$ & 12.93$_{\pm3.67}$ & 24.37$_{\pm5.30}$ & 9.41$_{\pm0.10}$ & 13.67$_{\pm4.33}$ & 10.26$_{\pm0.18}$ & 9.38$_{\pm0.12}$ & 10.30$_{\pm0.03}$ & \textbf{8.83$_{\pm0.05}$} \\
 &  & Avg & 8.75$_{\pm0.08}$ & 8.77$_{\pm0.06}$ & 8.68$_{\pm0.10}$ & 9.19$_{\pm0.15}$ & 20.89$_{\pm0.95}$ & 8.55$_{\pm0.09}$ & \underline{8.13$_{\pm0.07}$} & 8.25$_{\pm0.06}$ & 8.36$_{\pm0.19}$ & 8.70$_{\pm0.28}$ & 8.44$_{\pm0.14}$ & 12.02$_{\pm3.52}$ & 23.50$_{\pm5.70}$ & 8.55$_{\pm0.09}$ & 13.02$_{\pm4.40}$ & 9.54$_{\pm0.14}$ & 8.52$_{\pm0.14}$ & 8.95$_{\pm0.04}$ & \textbf{8.02$_{\pm0.06}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{RMSE} & 3 & 12.50$_{\pm0.16}$ & 12.08$_{\pm0.07}$ & 12.35$_{\pm0.13}$ & 12.58$_{\pm0.13}$ & 25.52$_{\pm1.03}$ & 11.98$_{\pm0.09}$ & \underline{11.52$_{\pm0.10}$} & 11.62$_{\pm0.09}$ & 11.80$_{\pm0.20}$ & 12.17$_{\pm0.43}$ & 11.89$_{\pm0.18}$ & 15.88$_{\pm3.26}$ & 31.12$_{\pm6.96}$ & 11.98$_{\pm0.09}$ & 17.90$_{\pm5.79}$ & 13.15$_{\pm0.21}$ & 11.96$_{\pm0.19}$ & 12.27$_{\pm0.06}$ & \textbf{11.31$_{\pm0.08}$} \\
 &  & 6 & 13.03$_{\pm0.12}$ & 13.25$_{\pm0.08}$ & 13.06$_{\pm0.11}$ & 13.49$_{\pm0.15}$ & 26.09$_{\pm1.03}$ & 12.86$_{\pm0.11}$ & \underline{12.21$_{\pm0.13}$} & 12.48$_{\pm0.06}$ & 12.58$_{\pm0.20}$ & 13.07$_{\pm0.40}$ & 12.70$_{\pm0.16}$ & 16.65$_{\pm3.37}$ & 31.67$_{\pm7.11}$ & 12.86$_{\pm0.11}$ & 18.44$_{\pm5.75}$ & 13.75$_{\pm0.21}$ & 12.87$_{\pm0.17}$ & 13.52$_{\pm0.06}$ & \textbf{12.20$_{\pm0.07}$} \\
 &  & 12 & 14.50$_{\pm0.11}$ & 15.55$_{\pm0.10}$ & 14.68$_{\pm0.13}$ & 15.69$_{\pm0.23}$ & 27.46$_{\pm1.18}$ & 14.65$_{\pm0.19}$ & \textbf{13.51$_{\pm0.19}$} & 14.07$_{\pm0.08}$ & 14.16$_{\pm0.21}$ & 14.87$_{\pm0.40}$ & 14.34$_{\pm0.19}$ & 18.24$_{\pm3.55}$ & 33.65$_{\pm6.61}$ & 14.65$_{\pm0.19}$ & 19.65$_{\pm5.68}$ & 15.02$_{\pm0.27}$ & 14.63$_{\pm0.16}$ & 16.09$_{\pm0.08}$ & \underline{13.80$_{\pm0.09}$} \\
 &  & Avg & 13.22$_{\pm0.13}$ & 13.42$_{\pm0.08}$ & 13.22$_{\pm0.12}$ & 13.75$_{\pm0.16}$ & 26.25$_{\pm1.04}$ & 13.01$_{\pm0.12}$ & \textbf{12.29$_{\pm0.13}$} & 12.58$_{\pm0.06}$ & 12.71$_{\pm0.20}$ & 13.21$_{\pm0.41}$ & 12.84$_{\pm0.17}$ & 16.78$_{\pm3.36}$ & 31.94$_{\pm6.92}$ & 13.01$_{\pm0.12}$ & 18.57$_{\pm5.76}$ & 13.86$_{\pm0.22}$ & 13.00$_{\pm0.17}$ & 13.74$_{\pm0.06}$ & \underline{12.29$_{\pm0.07}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{MAPE (\%)} & 3 & 33.99$_{\pm1.85}$ & 31.42$_{\pm1.45}$ & 35.07$_{\pm1.23}$ & 31.75$_{\pm1.62}$ & 287.97$_{\pm13.31}$ & 33.01$_{\pm1.29}$ & 30.28$_{\pm1.00}$ & \underline{29.57$_{\pm1.03}$} & 31.84$_{\pm2.12}$ & 34.22$_{\pm3.22}$ & 32.55$_{\pm1.67}$ & 91.33$_{\pm91.36}$ & 72.82$_{\pm24.46}$ & 33.01$_{\pm1.29}$ & 35.51$_{\pm3.14}$ & 52.45$_{\pm6.56}$ & 31.31$_{\pm1.84}$ & 32.31$_{\pm1.71}$ & \textbf{28.86$_{\pm0.78}$} \\
 &  & 6 & 34.37$_{\pm1.78}$ & 33.51$_{\pm1.51}$ & 35.88$_{\pm1.13}$ & 32.97$_{\pm1.44}$ & 288.59$_{\pm12.86}$ & 34.06$_{\pm1.17}$ & 31.34$_{\pm1.21}$ & \underline{30.32$_{\pm0.80}$} & 32.67$_{\pm2.60}$ & 35.22$_{\pm3.06}$ & 33.80$_{\pm1.47}$ & 91.86$_{\pm90.86}$ & 72.97$_{\pm21.57}$ & 34.06$_{\pm1.17}$ & 36.57$_{\pm3.25}$ & 53.80$_{\pm6.50}$ & 32.30$_{\pm1.83}$ & 34.60$_{\pm1.75}$ & \textbf{29.79$_{\pm0.71}$} \\
 &  & 12 & 36.05$_{\pm1.78}$ & 38.05$_{\pm1.43}$ & 38.74$_{\pm1.23}$ & 36.09$_{\pm1.00}$ & 292.23$_{\pm15.31}$ & 36.85$_{\pm1.36}$ & 33.80$_{\pm1.82}$ & \underline{32.43$_{\pm0.38}$} & 34.98$_{\pm3.34}$ & 37.80$_{\pm2.97}$ & 37.21$_{\pm1.53}$ & 96.41$_{\pm89.99}$ & 77.04$_{\pm16.92}$ & 36.85$_{\pm1.36}$ & 39.26$_{\pm3.27}$ & 57.37$_{\pm6.58}$ & 34.83$_{\pm1.61}$ & 40.50$_{\pm1.64}$ & \textbf{31.89$_{\pm0.70}$} \\
 &  & Avg & 34.68$_{\pm1.79}$ & 33.93$_{\pm1.44}$ & 36.32$_{\pm1.14}$ & 33.35$_{\pm1.40}$ & 289.51$_{\pm13.63}$ & 34.40$_{\pm1.24}$ & 31.58$_{\pm1.27}$ & \underline{30.57$_{\pm0.75}$} & 32.95$_{\pm2.62}$ & 35.53$_{\pm3.17}$ & 34.21$_{\pm1.55}$ & 92.72$_{\pm90.68}$ & 73.85$_{\pm20.96}$ & 34.40$_{\pm1.24}$ & 36.91$_{\pm3.18}$ & 54.23$_{\pm6.53}$ & 32.61$_{\pm1.76}$ & 35.31$_{\pm1.70}$ & \textbf{29.99$_{\pm0.72}$} \\
\midrule
\multirow{12}{*}{\textbf{PEMS06}} & \multirow{4}{*}{MAE} & 3 & 14.26$_{\pm2.99}$ & 10.47$_{\pm0.04}$ & 15.63$_{\pm0.10}$ & 11.17$_{\pm0.24}$ & 65.79$_{\pm1.35}$ & 10.13$_{\pm0.03}$ & 9.92$_{\pm0.10}$ & \underline{9.84$_{\pm0.12}$} & 9.98$_{\pm0.09}$ & 12.01$_{\pm3.14}$ & 10.39$_{\pm0.14}$ & 14.55$_{\pm3.45}$ & 45.96$_{\pm8.70}$ & 10.13$_{\pm0.03}$ & 49.20$_{\pm3.83}$ & 12.08$_{\pm0.21}$ & 10.36$_{\pm0.16}$ & 10.76$_{\pm0.07}$ & \textbf{9.58$_{\pm0.12}$} \\
 &  & 6 & 14.52$_{\pm3.01}$ & 11.33$_{\pm0.06}$ & 16.04$_{\pm0.09}$ & 11.87$_{\pm0.20}$ & 66.36$_{\pm1.17}$ & 10.76$_{\pm0.03}$ & 10.52$_{\pm0.13}$ & \underline{10.46$_{\pm0.17}$} & 10.62$_{\pm0.11}$ & 12.55$_{\pm3.06}$ & 10.99$_{\pm0.15}$ & 15.61$_{\pm3.25}$ & 45.52$_{\pm8.25}$ & 10.76$_{\pm0.03}$ & 49.25$_{\pm4.05}$ & 12.66$_{\pm0.18}$ & 10.98$_{\pm0.17}$ & 11.74$_{\pm0.06}$ & \textbf{10.26$_{\pm0.16}$} \\
 &  & 12 & 15.57$_{\pm2.98}$ & 13.10$_{\pm0.13}$ & 17.07$_{\pm0.09}$ & 13.48$_{\pm0.22}$ & 66.88$_{\pm1.23}$ & 12.06$_{\pm0.07}$ & 11.72$_{\pm0.20}$ & \underline{11.69$_{\pm0.24}$} & 11.87$_{\pm0.14}$ & 13.70$_{\pm2.90}$ & 12.30$_{\pm0.17}$ & 17.88$_{\pm2.88}$ & 43.40$_{\pm7.61}$ & 12.06$_{\pm0.07}$ & 49.72$_{\pm3.91}$ & 13.91$_{\pm0.19}$ & 12.32$_{\pm0.21}$ & 13.86$_{\pm0.04}$ & \textbf{11.52$_{\pm0.22}$} \\
 &  & Avg & 14.70$_{\pm3.00}$ & 11.47$_{\pm0.07}$ & 16.16$_{\pm0.09}$ & 12.04$_{\pm0.21}$ & 66.26$_{\pm1.22}$ & 10.86$_{\pm0.04}$ & 10.61$_{\pm0.14}$ & \underline{10.55$_{\pm0.17}$} & 10.71$_{\pm0.11}$ & 12.64$_{\pm3.05}$ & 11.10$_{\pm0.16}$ & 15.82$_{\pm3.21}$ & 45.05$_{\pm8.21}$ & 10.86$_{\pm0.04}$ & 49.34$_{\pm3.94}$ & 12.78$_{\pm0.19}$ & 11.10$_{\pm0.18}$ & 11.93$_{\pm0.06}$ & \textbf{10.34$_{\pm0.16}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{RMSE} & 3 & 20.17$_{\pm3.25}$ & 16.02$_{\pm0.07}$ & 24.68$_{\pm0.14}$ & 16.88$_{\pm0.41}$ & 81.19$_{\pm1.86}$ & 15.43$_{\pm0.05}$ & 15.16$_{\pm0.16}$ & \underline{14.95$_{\pm0.21}$} & 15.17$_{\pm0.15}$ & 18.87$_{\pm5.96}$ & 15.71$_{\pm0.21}$ & 20.88$_{\pm4.35}$ & 59.79$_{\pm11.67}$ & 15.43$_{\pm0.05}$ & 68.42$_{\pm4.46}$ & 17.65$_{\pm0.26}$ & 15.64$_{\pm0.14}$ & 16.51$_{\pm0.08}$ & \textbf{14.57$_{\pm0.18}$} \\
 &  & 6 & 20.78$_{\pm3.26}$ & 17.58$_{\pm0.11}$ & 25.44$_{\pm0.13}$ & 18.15$_{\pm0.33}$ & 82.22$_{\pm1.68}$ & 16.66$_{\pm0.03}$ & 16.34$_{\pm0.22}$ & \underline{16.16$_{\pm0.27}$} & 16.40$_{\pm0.17}$ & 19.87$_{\pm5.64}$ & 16.92$_{\pm0.21}$ & 22.76$_{\pm3.92}$ & 59.64$_{\pm10.69}$ & 16.66$_{\pm0.03}$ & 68.68$_{\pm4.72}$ & 18.59$_{\pm0.22}$ & 16.80$_{\pm0.16}$ & 18.32$_{\pm0.07}$ & \textbf{15.84$_{\pm0.23}$} \\
 &  & 12 & 22.72$_{\pm3.19}$ & 20.49$_{\pm0.22}$ & 27.18$_{\pm0.13}$ & 20.85$_{\pm0.28}$ & 83.64$_{\pm1.64}$ & 18.95$_{\pm0.10}$ & 18.48$_{\pm0.35}$ & \underline{18.37$_{\pm0.38}$} & 18.65$_{\pm0.23}$ & 21.80$_{\pm5.10}$ & 19.28$_{\pm0.23}$ & 26.57$_{\pm3.15}$ & 57.97$_{\pm9.46}$ & 18.95$_{\pm0.10}$ & 69.49$_{\pm4.56}$ & 20.58$_{\pm0.21}$ & 19.16$_{\pm0.24}$ & 21.83$_{\pm0.06}$ & \textbf{18.12$_{\pm0.33}$} \\
 &  & Avg & 21.06$_{\pm3.24}$ & 17.75$_{\pm0.12}$ & 25.62$_{\pm0.14}$ & 18.39$_{\pm0.34}$ & 82.15$_{\pm1.70}$ & 16.79$_{\pm0.04}$ & 16.45$_{\pm0.23}$ & \underline{16.29$_{\pm0.27}$} & 16.52$_{\pm0.17}$ & 19.99$_{\pm5.62}$ & 17.08$_{\pm0.21}$ & 23.08$_{\pm3.84}$ & 59.15$_{\pm10.67}$ & 16.79$_{\pm0.04}$ & 68.78$_{\pm4.59}$ & 18.77$_{\pm0.23}$ & 16.98$_{\pm0.17}$ & 18.56$_{\pm0.07}$ & \textbf{15.96$_{\pm0.24}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{MAPE (\%)} & 3 & 58.19$_{\pm29.81}$ & 22.49$_{\pm0.48}$ & 28.46$_{\pm1.67}$ & 24.59$_{\pm1.29}$ & 75.82$_{\pm2.75}$ & 23.24$_{\pm1.45}$ & \underline{21.21$_{\pm0.65}$} & 21.67$_{\pm0.66}$ & 21.90$_{\pm0.49}$ & 27.02$_{\pm7.14}$ & 25.97$_{\pm1.52}$ & 36.18$_{\pm18.89}$ & 67.56$_{\pm5.93}$ & 23.24$_{\pm1.45}$ & 50.16$_{\pm1.68}$ & 33.48$_{\pm2.54}$ & 24.85$_{\pm3.08}$ & 23.70$_{\pm1.11}$ & \textbf{20.80$_{\pm0.64}$} \\
 &  & 6 & 58.57$_{\pm29.86}$ & 23.77$_{\pm0.63}$ & 28.85$_{\pm1.65}$ & 25.64$_{\pm1.36}$ & 75.88$_{\pm3.01}$ & 24.13$_{\pm1.19}$ & \underline{21.92$_{\pm0.57}$} & 22.56$_{\pm0.65}$ & 22.51$_{\pm0.44}$ & 27.78$_{\pm7.06}$ & 26.48$_{\pm1.53}$ & 37.23$_{\pm18.98}$ & 69.33$_{\pm8.74}$ & 24.13$_{\pm1.19}$ & 50.11$_{\pm1.10}$ & 34.58$_{\pm2.73}$ & 25.84$_{\pm3.02}$ & 25.54$_{\pm1.17}$ & \textbf{21.72$_{\pm0.88}$} \\
 &  & 12 & 60.22$_{\pm29.91}$ & 27.09$_{\pm1.04}$ & 30.64$_{\pm1.69}$ & 28.30$_{\pm1.49}$ & 75.47$_{\pm3.01}$ & 26.52$_{\pm0.90}$ & \textbf{23.35$_{\pm0.67}$} & 24.51$_{\pm1.23}$ & 24.22$_{\pm0.51}$ & 29.63$_{\pm6.97}$ & 28.19$_{\pm1.50}$ & 39.35$_{\pm19.29}$ & 71.72$_{\pm17.59}$ & 26.52$_{\pm0.90}$ & 50.99$_{\pm1.07}$ & 37.39$_{\pm3.17}$ & 28.02$_{\pm3.11}$ & 30.02$_{\pm1.43}$ & \underline{23.39$_{\pm1.14}$} \\
 &  & Avg & 58.90$_{\pm29.90}$ & 24.15$_{\pm0.67}$ & 29.16$_{\pm1.65}$ & 25.94$_{\pm1.37}$ & 75.85$_{\pm2.88}$ & 24.41$_{\pm1.19}$ & \underline{22.03$_{\pm0.58}$} & 22.75$_{\pm0.79}$ & 22.72$_{\pm0.43}$ & 27.97$_{\pm7.04}$ & 26.68$_{\pm1.56}$ & 37.39$_{\pm19.08}$ & 69.42$_{\pm9.73}$ & 24.41$_{\pm1.19}$ & 50.35$_{\pm1.36}$ & 34.90$_{\pm2.77}$ & 26.03$_{\pm3.07}$ & 26.05$_{\pm1.22}$ & \textbf{21.82$_{\pm0.85}$} \\
\midrule
\multirow{12}{*}{\textbf{PEMS07}} & \multirow{4}{*}{MAE} & 3 & 63.07$_{\pm5.51}$ & 15.08$_{\pm0.18}$ & 126.15$_{\pm1.70}$ & 16.92$_{\pm1.42}$ & 40.98$_{\pm1.89}$ & 14.53$_{\pm0.20}$ & \textbf{13.57$_{\pm0.10}$} & 13.98$_{\pm0.21}$ & 13.81$_{\pm0.09}$ & 16.10$_{\pm1.56}$ & 13.89$_{\pm0.19}$ & 14.93$_{\pm0.39}$ & 43.42$_{\pm18.18}$ & 14.53$_{\pm0.20}$ & 15.06$_{\pm1.49}$ & 21.62$_{\pm1.24}$ & 14.69$_{\pm0.13}$ & 15.01$_{\pm0.12}$ & \underline{13.68$_{\pm0.13}$} \\
 &  & 6 & 63.36$_{\pm5.45}$ & 16.76$_{\pm0.15}$ & 126.34$_{\pm1.70}$ & 17.81$_{\pm1.18}$ & 41.13$_{\pm1.62}$ & 15.86$_{\pm0.14}$ & \textbf{14.75$_{\pm0.11}$} & 15.39$_{\pm0.22}$ & 15.14$_{\pm0.10}$ & 17.34$_{\pm1.47}$ & 15.25$_{\pm0.17}$ & 15.87$_{\pm0.37}$ & 47.40$_{\pm20.15}$ & 15.86$_{\pm0.14}$ & 15.91$_{\pm1.42}$ & 23.50$_{\pm1.35}$ & 16.03$_{\pm0.14}$ & 16.89$_{\pm0.07}$ & \underline{15.14$_{\pm0.16}$} \\
 &  & 12 & 64.80$_{\pm5.38}$ & 20.43$_{\pm0.16}$ & 126.74$_{\pm1.64}$ & 20.20$_{\pm1.10}$ & 41.26$_{\pm1.68}$ & 18.48$_{\pm0.14}$ & \textbf{16.82$_{\pm0.17}$} & 17.92$_{\pm0.22}$ & \underline{17.54$_{\pm0.19}$} & 19.63$_{\pm1.34}$ & 17.72$_{\pm0.15}$ & 17.77$_{\pm0.44}$ & 58.50$_{\pm27.96}$ & 18.48$_{\pm0.14}$ & 18.38$_{\pm1.52}$ & 27.74$_{\pm1.60}$ & 18.74$_{\pm0.16}$ & 20.97$_{\pm0.06}$ & 17.76$_{\pm0.17}$ \\
 &  & Avg & 63.62$_{\pm5.47}$ & 17.10$_{\pm0.16}$ & 126.38$_{\pm1.68}$ & 18.10$_{\pm1.24}$ & 41.08$_{\pm1.72}$ & 16.04$_{\pm0.15}$ & \textbf{14.84$_{\pm0.12}$} & 15.52$_{\pm0.21}$ & \underline{15.27$_{\pm0.11}$} & 17.47$_{\pm1.47}$ & 15.38$_{\pm0.17}$ & 16.00$_{\pm0.38}$ & 48.98$_{\pm21.82}$ & 16.04$_{\pm0.15}$ & 16.23$_{\pm1.45}$ & 23.95$_{\pm1.37}$ & 16.23$_{\pm0.14}$ & 17.26$_{\pm0.08}$ & 15.28$_{\pm0.15}$ \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{RMSE} & 3 & 89.39$_{\pm6.03}$ & 24.87$_{\pm0.26}$ & 207.14$_{\pm1.48}$ & 27.20$_{\pm1.90}$ & 51.60$_{\pm1.77}$ & 23.85$_{\pm0.22}$ & \textbf{22.69$_{\pm0.10}$} & 23.21$_{\pm0.23}$ & 22.96$_{\pm0.12}$ & 25.78$_{\pm2.44}$ & 23.10$_{\pm0.21}$ & 24.22$_{\pm0.50}$ & 62.01$_{\pm24.03}$ & 23.85$_{\pm0.22}$ & 25.05$_{\pm2.32}$ & 34.19$_{\pm1.53}$ & 24.09$_{\pm0.08}$ & 25.12$_{\pm0.08}$ & \underline{22.92$_{\pm0.14}$} \\
 &  & 6 & 89.94$_{\pm6.01}$ & 27.95$_{\pm0.22}$ & 207.04$_{\pm1.49}$ & 28.79$_{\pm1.50}$ & 52.70$_{\pm1.41}$ & 26.35$_{\pm0.16}$ & \textbf{24.82$_{\pm0.15}$} & 25.69$_{\pm0.25}$ & \underline{25.39$_{\pm0.15}$} & 28.03$_{\pm2.21}$ & 25.54$_{\pm0.19}$ & 26.02$_{\pm0.46}$ & 69.43$_{\pm27.92}$ & 26.35$_{\pm0.16}$ & 26.46$_{\pm2.25}$ & 37.19$_{\pm1.52}$ & 26.49$_{\pm0.11}$ & 28.68$_{\pm0.07}$ & 25.47$_{\pm0.20}$ \\
 &  & 12 & 92.24$_{\pm5.89}$ & 34.29$_{\pm0.29}$ & 206.82$_{\pm1.46}$ & 32.78$_{\pm1.42}$ & 54.33$_{\pm1.42}$ & 30.92$_{\pm0.21}$ & \textbf{28.33$_{\pm0.25}$} & 29.90$_{\pm0.25}$ & 29.44$_{\pm0.26}$ & 31.97$_{\pm1.92}$ & 29.65$_{\pm0.20}$ & \underline{29.15$_{\pm0.64}$} & 88.34$_{\pm41.51}$ & 30.92$_{\pm0.21}$ & 30.31$_{\pm2.38}$ & 44.26$_{\pm1.57}$ & 31.02$_{\pm0.13}$ & 35.79$_{\pm0.10}$ & 29.79$_{\pm0.20}$ \\
 &  & Avg & 90.32$_{\pm6.01}$ & 28.45$_{\pm0.24}$ & 207.02$_{\pm1.47}$ & 29.22$_{\pm1.59}$ & 52.68$_{\pm1.51}$ & 26.60$_{\pm0.18}$ & \textbf{24.91$_{\pm0.15}$} & 25.84$_{\pm0.24}$ & \underline{25.52$_{\pm0.15}$} & 28.21$_{\pm2.23}$ & 25.68$_{\pm0.20}$ & 26.13$_{\pm0.50}$ & 71.90$_{\pm30.60}$ & 26.60$_{\pm0.18}$ & 26.89$_{\pm2.29}$ & 37.97$_{\pm1.51}$ & 26.76$_{\pm0.10}$ & 29.20$_{\pm0.07}$ & 25.62$_{\pm0.17}$ \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{MAPE (\%)} & 3 & 227.57$_{\pm91.05}$ & 18.75$_{\pm0.39}$ & 55.74$_{\pm1.64}$ & 20.66$_{\pm1.85}$ & 42.64$_{\pm1.49}$ & 18.95$_{\pm0.87}$ & 17.91$_{\pm0.37}$ & 18.00$_{\pm0.38}$ & \underline{17.45$_{\pm0.64}$} & 20.72$_{\pm1.55}$ & 17.57$_{\pm0.69}$ & 20.65$_{\pm1.03}$ & 55.23$_{\pm18.16}$ & 18.95$_{\pm0.87}$ & 21.64$_{\pm3.06}$ & 39.89$_{\pm2.72}$ & 19.54$_{\pm0.55}$ & 18.08$_{\pm0.57}$ & \textbf{17.14$_{\pm0.35}$} \\
 &  & 6 & 227.77$_{\pm90.51}$ & 20.21$_{\pm0.42}$ & 56.28$_{\pm1.56}$ & 21.45$_{\pm1.68}$ & 41.89$_{\pm1.52}$ & 20.03$_{\pm0.90}$ & 18.78$_{\pm0.43}$ & 18.98$_{\pm0.45}$ & \underline{18.49$_{\pm0.66}$} & 21.65$_{\pm1.56}$ & 18.70$_{\pm0.61}$ & 21.81$_{\pm1.31}$ & 57.38$_{\pm18.64}$ & 20.03$_{\pm0.90}$ & 22.66$_{\pm3.18}$ & 42.65$_{\pm3.25}$ & 20.57$_{\pm0.51}$ & 19.76$_{\pm0.55}$ & \textbf{18.10$_{\pm0.35}$} \\
 &  & 12 & 229.22$_{\pm90.29}$ & 24.00$_{\pm0.40}$ & 57.77$_{\pm1.40}$ & 23.99$_{\pm1.58}$ & 40.94$_{\pm2.06}$ & 22.56$_{\pm1.06}$ & 20.88$_{\pm0.78}$ & 21.24$_{\pm0.55}$ & \underline{20.84$_{\pm0.79}$} & 23.76$_{\pm1.63}$ & 21.32$_{\pm0.74}$ & 24.48$_{\pm1.71}$ & 63.85$_{\pm21.03}$ & 22.56$_{\pm1.06}$ & 26.08$_{\pm3.62}$ & 49.11$_{\pm4.41}$ & 23.04$_{\pm0.47}$ & 24.21$_{\pm0.74}$ & \textbf{20.09$_{\pm0.39}$} \\
 &  & Avg & 228.08$_{\pm90.59}$ & 20.65$_{\pm0.40}$ & 56.47$_{\pm1.53}$ & 21.82$_{\pm1.71}$ & 41.90$_{\pm1.61}$ & 20.30$_{\pm0.91}$ & 19.00$_{\pm0.48}$ & 19.20$_{\pm0.41}$ & \underline{18.73$_{\pm0.69}$} & 21.85$_{\pm1.56}$ & 18.97$_{\pm0.67}$ & 22.09$_{\pm1.19}$ & 58.27$_{\pm19.00}$ & 20.30$_{\pm0.91}$ & 23.17$_{\pm3.24}$ & 43.38$_{\pm3.34}$ & 20.83$_{\pm0.48}$ & 20.31$_{\pm0.60}$ & \textbf{18.26$_{\pm0.36}$} \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> table/newsensor2.tex <==
\begin{table*}[t]
\centering
\caption{Newly-added-sensor forecast errors, part 2/2 (PEMS08, PEMS10, PEMS11, PEMS12; mean$\pm$std over seeds per dataset). Years where the graph did not grow are excluded. Baselines are grouped and ordered to match \Cref{tab:main_full}. \textbf{Bold}: best, \underline{underline}: second best.}
\label{tab:tsas_new_sensors_part2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccc|cccc|cccc|cccc|cc|cccc|c}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metric}} & \multirow{2}{*}{\textbf{Horizon}} & \multicolumn{4}{c|}{\textbf{Static STGNN Backbones}} & \multicolumn{4}{c|}{\textbf{Na\"ive Schemes}} & \multicolumn{4}{c|}{\textbf{Evolving-Graph Continual}} & \multicolumn{2}{c|}{\textbf{Retrieval / TTC}} & \multicolumn{4}{c|}{\textbf{Other Static Backbones}} & \multicolumn{1}{c}{\textbf{Ours}} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-11} \cmidrule(lr){12-15} \cmidrule(lr){16-17} \cmidrule(lr){18-21} \cmidrule(lr){22-22}
 &  &  & \textbf{DCRNN} & \textbf{ASTGNN} & \textbf{TGCN} & \textbf{GWN} & \textbf{Pretrain} & \textbf{Retrain} & \textbf{OL-NN} & \textbf{OL-AN} & \textbf{TrafStm} & \textbf{PECPM} & \textbf{STKEC} & \textbf{EAC} & \textbf{STRAP} & \textbf{ST-TTC} & \textbf{STID} & \textbf{STNorm} & \textbf{iTrans} & \textbf{DLinear} & \textbf{A2TTA} \\
\midrule
\multirow{12}{*}{\textbf{PEMS08}} & \multirow{4}{*}{MAE} & 3 & 63.20$_{\pm14.64}$ & 13.94$_{\pm0.08}$ & 90.82$_{\pm1.78}$ & 15.12$_{\pm0.38}$ & 56.25$_{\pm2.73}$ & 13.52$_{\pm0.08}$ & \underline{12.86$_{\pm0.08}$} & 13.03$_{\pm0.13}$ & 12.97$_{\pm0.12}$ & 15.08$_{\pm0.90}$ & 13.58$_{\pm0.57}$ & 14.37$_{\pm0.25}$ & 38.43$_{\pm9.73}$ & 13.52$_{\pm0.08}$ & 111.42$_{\pm3.40}$ & 17.00$_{\pm0.42}$ & 13.76$_{\pm0.03}$ & 14.06$_{\pm0.04}$ & \textbf{12.72$_{\pm0.09}$} \\
 &  & 6 & 63.50$_{\pm14.64}$ & 15.34$_{\pm0.08}$ & 91.03$_{\pm1.77}$ & 15.98$_{\pm0.25}$ & 56.02$_{\pm2.83}$ & 14.61$_{\pm0.06}$ & \underline{13.94$_{\pm0.11}$} & 14.16$_{\pm0.11}$ & 14.08$_{\pm0.13}$ & 16.04$_{\pm0.85}$ & 14.58$_{\pm0.43}$ & 15.21$_{\pm0.22}$ & 39.83$_{\pm9.50}$ & 14.61$_{\pm0.06}$ & 111.70$_{\pm2.79}$ & 18.02$_{\pm0.34}$ & 14.86$_{\pm0.04}$ & 15.61$_{\pm0.02}$ & \textbf{13.88$_{\pm0.10}$} \\
 &  & 12 & 64.57$_{\pm14.44}$ & 18.35$_{\pm0.12}$ & 91.63$_{\pm1.74}$ & 18.28$_{\pm0.15}$ & 55.80$_{\pm3.30}$ & 16.83$_{\pm0.06}$ & \textbf{15.90$_{\pm0.18}$} & 16.23$_{\pm0.11}$ & 16.12$_{\pm0.17}$ & 17.86$_{\pm0.73}$ & 16.59$_{\pm0.38}$ & 16.86$_{\pm0.21}$ & 43.52$_{\pm9.63}$ & 16.83$_{\pm0.06}$ & 111.84$_{\pm2.57}$ & 20.39$_{\pm0.42}$ & 17.03$_{\pm0.08}$ & 18.95$_{\pm0.04}$ & \underline{15.99$_{\pm0.12}$} \\
 &  & Avg & 63.68$_{\pm14.57}$ & 15.61$_{\pm0.08}$ & 91.11$_{\pm1.77}$ & 16.27$_{\pm0.26}$ & 56.03$_{\pm2.93}$ & 14.79$_{\pm0.07}$ & \underline{14.05$_{\pm0.12}$} & 14.28$_{\pm0.11}$ & 14.20$_{\pm0.14}$ & 16.15$_{\pm0.84}$ & 14.73$_{\pm0.47}$ & 15.31$_{\pm0.22}$ & 40.32$_{\pm9.56}$ & 14.79$_{\pm0.07}$ & 111.83$_{\pm2.82}$ & 18.28$_{\pm0.35}$ & 15.02$_{\pm0.04}$ & 15.91$_{\pm0.02}$ & \textbf{14.00$_{\pm0.10}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{RMSE} & 3 & 81.62$_{\pm17.23}$ & 22.93$_{\pm0.13}$ & 138.77$_{\pm3.38}$ & 23.91$_{\pm0.47}$ & 65.76$_{\pm3.15}$ & 22.14$_{\pm0.10}$ & \underline{21.30$_{\pm0.09}$} & 21.54$_{\pm0.15}$ & 21.43$_{\pm0.13}$ & 24.01$_{\pm1.20}$ & 22.12$_{\pm0.63}$ & 22.77$_{\pm0.31}$ & 52.13$_{\pm12.73}$ & 22.14$_{\pm0.10}$ & 170.06$_{\pm3.34}$ & 25.96$_{\pm0.52}$ & 22.46$_{\pm0.06}$ & 23.19$_{\pm0.04}$ & \textbf{21.19$_{\pm0.10}$} \\
 &  & 6 & 82.29$_{\pm17.12}$ & 25.57$_{\pm0.13}$ & 139.03$_{\pm3.34}$ & 25.67$_{\pm0.25}$ & 66.21$_{\pm3.21}$ & 24.36$_{\pm0.09}$ & \textbf{23.36$_{\pm0.16}$} & 23.76$_{\pm0.13}$ & 23.64$_{\pm0.16}$ & 25.96$_{\pm1.07}$ & 24.19$_{\pm0.46}$ & 24.47$_{\pm0.28}$ & 55.04$_{\pm12.48}$ & 24.36$_{\pm0.09}$ & 170.32$_{\pm2.96}$ & 27.68$_{\pm0.44}$ & 24.59$_{\pm0.07}$ & 26.15$_{\pm0.03}$ & \underline{23.45$_{\pm0.10}$} \\
 &  & 12 & 84.13$_{\pm16.66}$ & 30.71$_{\pm0.18}$ & 139.63$_{\pm3.25}$ & 29.71$_{\pm0.18}$ & 67.30$_{\pm3.67}$ & 28.47$_{\pm0.12}$ & \textbf{26.88$_{\pm0.32}$} & 27.55$_{\pm0.15}$ & 27.39$_{\pm0.29}$ & 29.45$_{\pm0.85}$ & 27.99$_{\pm0.57}$ & 27.43$_{\pm0.35}$ & 61.94$_{\pm13.05}$ & 28.47$_{\pm0.12}$ & 170.24$_{\pm2.53}$ & 31.57$_{\pm0.64}$ & 28.49$_{\pm0.12}$ & 31.98$_{\pm0.05}$ & \underline{27.31$_{\pm0.13}$} \\
 &  & Avg & 82.53$_{\pm17.02}$ & 25.93$_{\pm0.14}$ & 139.08$_{\pm3.34}$ & 26.08$_{\pm0.28}$ & 66.31$_{\pm3.32}$ & 24.61$_{\pm0.10}$ & \textbf{23.51$_{\pm0.17}$} & 23.92$_{\pm0.14}$ & 23.80$_{\pm0.18}$ & 26.15$_{\pm1.06}$ & 24.41$_{\pm0.55}$ & 24.59$_{\pm0.31}$ & 55.82$_{\pm12.59}$ & 24.61$_{\pm0.10}$ & 170.39$_{\pm2.80}$ & 28.08$_{\pm0.46}$ & 24.82$_{\pm0.07}$ & 26.58$_{\pm0.02}$ & \underline{23.62$_{\pm0.11}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{MAPE (\%)} & 3 & 316.71$_{\pm89.09}$ & 19.29$_{\pm0.28}$ & 58.18$_{\pm1.88}$ & 21.67$_{\pm1.92}$ & 58.26$_{\pm1.28}$ & 20.17$_{\pm0.82}$ & 18.65$_{\pm0.43}$ & \underline{18.36$_{\pm0.18}$} & 19.24$_{\pm0.78}$ & 22.52$_{\pm1.95}$ & 20.80$_{\pm1.74}$ & 26.09$_{\pm1.75}$ & 56.67$_{\pm13.14}$ & 20.17$_{\pm0.82}$ & 53.03$_{\pm1.94}$ & 36.11$_{\pm4.54}$ & 21.46$_{\pm0.77}$ & 18.99$_{\pm0.56}$ & \textbf{17.31$_{\pm0.36}$} \\
 &  & 6 & 317.48$_{\pm89.04}$ & 20.71$_{\pm0.32}$ & 58.58$_{\pm1.82}$ & 22.51$_{\pm1.91}$ & 57.75$_{\pm1.78}$ & 21.23$_{\pm0.70}$ & 19.77$_{\pm0.47}$ & \underline{19.38$_{\pm0.30}$} & 20.33$_{\pm0.73}$ & 23.54$_{\pm1.91}$ & 21.77$_{\pm1.54}$ & 26.29$_{\pm1.62}$ & 59.45$_{\pm13.27}$ & 21.23$_{\pm0.70}$ & 53.27$_{\pm1.87}$ & 37.52$_{\pm4.50}$ & 22.55$_{\pm0.74}$ & 20.65$_{\pm0.50}$ & \textbf{18.20$_{\pm0.36}$} \\
 &  & 12 & 318.88$_{\pm88.78}$ & 24.18$_{\pm0.54}$ & 60.00$_{\pm1.72}$ & 25.09$_{\pm1.86}$ & 57.48$_{\pm2.77}$ & 23.76$_{\pm0.52}$ & 22.30$_{\pm0.69}$ & \underline{21.86$_{\pm0.39}$} & 22.85$_{\pm0.67}$ & 25.75$_{\pm1.86}$ & 23.98$_{\pm1.05}$ & 27.74$_{\pm2.25}$ & 66.63$_{\pm13.58}$ & 23.76$_{\pm0.52}$ & 54.62$_{\pm1.86}$ & 41.10$_{\pm4.52}$ & 25.07$_{\pm0.73}$ & 24.82$_{\pm0.61}$ & \textbf{20.04$_{\pm0.34}$} \\
 &  & Avg & 317.57$_{\pm88.99}$ & 21.08$_{\pm0.34}$ & 58.82$_{\pm1.84}$ & 22.87$_{\pm1.90}$ & 57.92$_{\pm1.82}$ & 21.50$_{\pm0.66}$ & 20.02$_{\pm0.50}$ & \underline{19.66$_{\pm0.26}$} & 20.59$_{\pm0.70}$ & 23.74$_{\pm1.90}$ & 22.00$_{\pm1.45}$ & 26.54$_{\pm1.50}$ & 60.35$_{\pm13.14}$ & 21.50$_{\pm0.66}$ & 53.59$_{\pm1.75}$ & 37.96$_{\pm4.51}$ & 22.83$_{\pm0.72}$ & 21.14$_{\pm0.52}$ & \textbf{18.36$_{\pm0.35}$} \\
\midrule
\multirow{12}{*}{\textbf{PEMS10}} & \multirow{4}{*}{MAE} & 3 & 10.50$_{\pm0.21}$ & 9.95$_{\pm0.05}$ & 10.98$_{\pm0.07}$ & 10.41$_{\pm0.16}$ & 83.95$_{\pm3.34}$ & 9.69$_{\pm0.06}$ & \textbf{9.39$_{\pm0.09}$} & 9.56$_{\pm0.05}$ & 9.70$_{\pm0.09}$ & 10.45$_{\pm1.00}$ & 9.73$_{\pm0.09}$ & 11.59$_{\pm1.92}$ & 25.66$_{\pm3.68}$ & 9.69$_{\pm0.06}$ & 10.43$_{\pm0.13}$ & 11.42$_{\pm0.26}$ & 9.78$_{\pm0.07}$ & 10.10$_{\pm0.05}$ & \underline{9.41$_{\pm0.04}$} \\
 &  & 6 & 10.74$_{\pm0.17}$ & 10.69$_{\pm0.03}$ & 11.37$_{\pm0.06}$ & 10.85$_{\pm0.17}$ & 84.23$_{\pm3.40}$ & 10.25$_{\pm0.06}$ & \textbf{9.90$_{\pm0.14}$} & 10.13$_{\pm0.07}$ & 10.26$_{\pm0.11}$ & 10.96$_{\pm0.93}$ & 10.26$_{\pm0.09}$ & 12.13$_{\pm2.00}$ & 25.94$_{\pm4.48}$ & 10.25$_{\pm0.06}$ & 10.90$_{\pm0.11}$ & 11.84$_{\pm0.28}$ & 10.32$_{\pm0.07}$ & 10.92$_{\pm0.05}$ & \underline{9.98$_{\pm0.05}$} \\
 &  & 12 & 11.74$_{\pm0.17}$ & 12.23$_{\pm0.02}$ & 12.38$_{\pm0.06}$ & 12.01$_{\pm0.22}$ & 84.43$_{\pm3.39}$ & 11.43$_{\pm0.04}$ & \textbf{10.92$_{\pm0.23}$} & 11.26$_{\pm0.09}$ & 11.44$_{\pm0.15}$ & 12.05$_{\pm0.84}$ & 11.38$_{\pm0.11}$ & 13.42$_{\pm2.24}$ & 29.38$_{\pm9.77}$ & 11.43$_{\pm0.04}$ & 12.12$_{\pm0.13}$ & 12.88$_{\pm0.32}$ & 11.44$_{\pm0.09}$ & 12.71$_{\pm0.05}$ & \underline{11.13$_{\pm0.06}$} \\
 &  & Avg & 10.92$_{\pm0.18}$ & 10.82$_{\pm0.03}$ & 11.50$_{\pm0.06}$ & 10.99$_{\pm0.18}$ & 84.20$_{\pm3.29}$ & 10.36$_{\pm0.05}$ & \textbf{9.98$_{\pm0.15}$} & 10.22$_{\pm0.07}$ & 10.37$_{\pm0.11}$ & 11.06$_{\pm0.93}$ & 10.36$_{\pm0.09}$ & 12.27$_{\pm2.03}$ & 26.73$_{\pm5.48}$ & 10.36$_{\pm0.05}$ & 11.04$_{\pm0.12}$ & 11.96$_{\pm0.27}$ & 10.41$_{\pm0.07}$ & 11.09$_{\pm0.05}$ & \underline{10.07$_{\pm0.05}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{RMSE} & 3 & 16.84$_{\pm0.44}$ & 16.00$_{\pm0.11}$ & 19.16$_{\pm0.16}$ & 16.54$_{\pm0.19}$ & 86.11$_{\pm3.42}$ & 15.46$_{\pm0.09}$ & \underline{15.03$_{\pm0.15}$} & 15.23$_{\pm0.09}$ & 15.47$_{\pm0.11}$ & 17.13$_{\pm2.26}$ & 15.54$_{\pm0.10}$ & 17.21$_{\pm1.72}$ & 35.95$_{\pm5.42}$ & 15.46$_{\pm0.09}$ & 16.56$_{\pm0.20}$ & 17.70$_{\pm0.40}$ & 15.65$_{\pm0.13}$ & 16.19$_{\pm0.06}$ & \textbf{15.00$_{\pm0.06}$} \\
 &  & 6 & 17.43$_{\pm0.38}$ & 17.37$_{\pm0.08}$ & 19.87$_{\pm0.15}$ & 17.41$_{\pm0.21}$ & 86.77$_{\pm3.55}$ & 16.58$_{\pm0.09}$ & \textbf{16.03$_{\pm0.24}$} & 16.36$_{\pm0.13}$ & 16.57$_{\pm0.16}$ & 18.14$_{\pm2.09}$ & 16.61$_{\pm0.12}$ & 18.26$_{\pm1.75}$ & 37.22$_{\pm7.11}$ & 16.58$_{\pm0.09}$ & 17.44$_{\pm0.16}$ & 18.45$_{\pm0.46}$ & 16.71$_{\pm0.14}$ & 17.71$_{\pm0.06}$ & \underline{16.12$_{\pm0.09}$} \\
 &  & 12 & 19.30$_{\pm0.38}$ & 20.05$_{\pm0.05}$ & 21.60$_{\pm0.14}$ & 19.46$_{\pm0.30}$ & 87.72$_{\pm3.63}$ & 18.82$_{\pm0.06}$ & \textbf{17.92$_{\pm0.43}$} & 18.53$_{\pm0.15}$ & 18.75$_{\pm0.26}$ & 20.14$_{\pm1.80}$ & 18.74$_{\pm0.16}$ & 20.43$_{\pm1.96}$ & 43.59$_{\pm15.75}$ & 18.82$_{\pm0.06}$ & 19.48$_{\pm0.19}$ & 20.22$_{\pm0.56}$ & 18.80$_{\pm0.14}$ & 20.80$_{\pm0.06}$ & \underline{18.35$_{\pm0.12}$} \\
 &  & Avg & 17.71$_{\pm0.40}$ & 17.57$_{\pm0.07}$ & 20.07$_{\pm0.15}$ & 17.63$_{\pm0.22}$ & 86.80$_{\pm3.44}$ & 16.76$_{\pm0.08}$ & \textbf{16.16$_{\pm0.26}$} & 16.51$_{\pm0.12}$ & 16.75$_{\pm0.17}$ & 18.30$_{\pm2.08}$ & 16.78$_{\pm0.12}$ & 18.43$_{\pm1.78}$ & 38.41$_{\pm8.72}$ & 16.76$_{\pm0.08}$ & 17.65$_{\pm0.18}$ & 18.64$_{\pm0.45}$ & 16.87$_{\pm0.14}$ & 17.97$_{\pm0.06}$ & \underline{16.29$_{\pm0.08}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{MAPE (\%)} & 3 & 32.35$_{\pm0.71}$ & 29.97$_{\pm0.78}$ & 31.64$_{\pm0.79}$ & 31.72$_{\pm1.66}$ & 948.50$_{\pm34.27}$ & 31.31$_{\pm1.00}$ & \textbf{29.29$_{\pm0.39}$} & 30.84$_{\pm0.47}$ & 32.37$_{\pm0.81}$ & 31.02$_{\pm1.72}$ & 31.31$_{\pm0.60}$ & 66.78$_{\pm48.94}$ & 138.67$_{\pm35.18}$ & 31.31$_{\pm1.00}$ & 34.71$_{\pm0.85}$ & 44.44$_{\pm2.05}$ & 30.94$_{\pm1.15}$ & 30.48$_{\pm0.68}$ & \underline{29.40$_{\pm0.32}$} \\
 &  & 6 & 33.04$_{\pm0.67}$ & 31.54$_{\pm0.81}$ & 32.45$_{\pm0.79}$ & 32.65$_{\pm1.62}$ & 946.34$_{\pm33.65}$ & 32.39$_{\pm1.03}$ & \underline{30.34$_{\pm0.53}$} & 31.69$_{\pm0.38}$ & 33.62$_{\pm0.84}$ & 32.01$_{\pm1.68}$ & 32.39$_{\pm0.72}$ & 67.39$_{\pm50.04}$ & 131.51$_{\pm31.92}$ & 32.39$_{\pm1.03}$ & 35.94$_{\pm0.78}$ & 45.66$_{\pm2.03}$ & 31.97$_{\pm1.33}$ & 32.50$_{\pm0.62}$ & \textbf{30.23$_{\pm0.27}$} \\
 &  & 12 & 35.48$_{\pm0.77}$ & 35.40$_{\pm0.87}$ & 35.14$_{\pm0.83}$ & 35.43$_{\pm1.66}$ & 941.79$_{\pm29.53}$ & 35.20$_{\pm1.09}$ & \underline{32.87$_{\pm1.09}$} & 34.31$_{\pm0.49}$ & 37.22$_{\pm0.96}$ & 34.78$_{\pm1.67}$ & 35.01$_{\pm0.81}$ & 71.78$_{\pm53.06}$ & 132.50$_{\pm33.98}$ & 35.20$_{\pm1.09}$ & 39.44$_{\pm0.83}$ & 48.96$_{\pm2.05}$ & 34.53$_{\pm1.67}$ & 37.55$_{\pm0.56}$ & \textbf{32.22$_{\pm0.27}$} \\
 &  & Avg & 33.42$_{\pm0.71}$ & 31.97$_{\pm0.80}$ & 32.85$_{\pm0.79}$ & 33.04$_{\pm1.64}$ & 946.03$_{\pm32.27}$ & 32.75$_{\pm1.02}$ & \underline{30.64$_{\pm0.61}$} & 32.07$_{\pm0.40}$ & 34.11$_{\pm0.80}$ & 32.38$_{\pm1.68}$ & 32.71$_{\pm0.68}$ & 68.33$_{\pm50.45}$ & 134.18$_{\pm32.27}$ & 32.75$_{\pm1.02}$ & 36.39$_{\pm0.79}$ & 46.09$_{\pm2.03}$ & 32.26$_{\pm1.35}$ & 33.09$_{\pm0.60}$ & \textbf{30.45$_{\pm0.27}$} \\
\midrule
\multirow{12}{*}{\textbf{PEMS11}} & \multirow{4}{*}{MAE} & 3 & 52.60$_{\pm9.32}$ & 16.96$_{\pm0.10}$ & 84.02$_{\pm5.17}$ & 18.47$_{\pm0.48}$ & 87.20$_{\pm3.86}$ & 16.41$_{\pm0.21}$ & \underline{15.91$_{\pm0.16}$} & 15.97$_{\pm0.27}$ & 16.27$_{\pm0.19}$ & 24.70$_{\pm3.26}$ & 17.02$_{\pm0.32}$ & 23.34$_{\pm3.67}$ & 56.94$_{\pm10.89}$ & 16.41$_{\pm0.21}$ & 16.42$_{\pm2.92}$ & 20.16$_{\pm0.67}$ & 16.66$_{\pm0.29}$ & 17.22$_{\pm0.16}$ & \textbf{15.26$_{\pm0.17}$} \\
 &  & 6 & 53.24$_{\pm9.23}$ & 18.93$_{\pm0.08}$ & 84.14$_{\pm5.16}$ & 19.65$_{\pm0.48}$ & 88.94$_{\pm3.54}$ & 18.09$_{\pm0.16}$ & 17.52$_{\pm0.21}$ & 17.69$_{\pm0.23}$ & 18.02$_{\pm0.16}$ & 26.11$_{\pm3.10}$ & 18.73$_{\pm0.20}$ & 25.02$_{\pm4.08}$ & 58.28$_{\pm10.35}$ & 18.09$_{\pm0.16}$ & \underline{17.41$_{\pm2.98}$} & 21.69$_{\pm0.82}$ & 18.32$_{\pm0.24}$ & 19.30$_{\pm0.11}$ & \textbf{17.06$_{\pm0.13}$} \\
 &  & 12 & 55.51$_{\pm9.05}$ & 23.17$_{\pm0.15}$ & 84.89$_{\pm5.06}$ & 22.82$_{\pm0.72}$ & 92.59$_{\pm3.19}$ & 21.58$_{\pm0.17}$ & 20.73$_{\pm0.31}$ & 20.99$_{\pm0.20}$ & 21.48$_{\pm0.22}$ & 29.03$_{\pm2.86}$ & 22.20$_{\pm0.22}$ & 29.10$_{\pm4.48}$ & 62.94$_{\pm8.34}$ & 21.58$_{\pm0.17}$ & \textbf{20.16$_{\pm3.22}$} & 24.84$_{\pm1.26}$ & 21.85$_{\pm0.21}$ & 23.94$_{\pm0.11}$ & \underline{20.51$_{\pm0.12}$} \\
 &  & Avg & 53.61$_{\pm9.22}$ & 19.32$_{\pm0.09}$ & 84.29$_{\pm5.14}$ & 20.05$_{\pm0.52}$ & 89.25$_{\pm3.53}$ & 18.39$_{\pm0.17}$ & \underline{17.77$_{\pm0.21}$} & 17.92$_{\pm0.24}$ & 18.29$_{\pm0.19}$ & 26.35$_{\pm3.09}$ & 19.02$_{\pm0.22}$ & 25.48$_{\pm4.02}$ & 59.09$_{\pm9.67}$ & 18.39$_{\pm0.17}$ & 17.77$_{\pm3.02}$ & 21.98$_{\pm0.83}$ & 18.64$_{\pm0.25}$ & 19.76$_{\pm0.13}$ & \textbf{17.31$_{\pm0.15}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{RMSE} & 3 & 70.68$_{\pm11.75}$ & 26.86$_{\pm0.22}$ & 131.75$_{\pm6.52}$ & 28.77$_{\pm0.66}$ & 110.71$_{\pm3.46}$ & 25.77$_{\pm0.21}$ & \underline{25.09$_{\pm0.15}$} & 25.19$_{\pm0.27}$ & 25.47$_{\pm0.27}$ & 39.42$_{\pm6.00}$ & 26.42$_{\pm0.25}$ & 34.80$_{\pm4.82}$ & 75.77$_{\pm13.30}$ & 25.77$_{\pm0.21}$ & 25.10$_{\pm3.99}$ & 30.89$_{\pm0.73}$ & 26.02$_{\pm0.35}$ & 27.31$_{\pm0.15}$ & \textbf{24.23$_{\pm0.17}$} \\
 &  & 6 & 72.15$_{\pm11.55}$ & 30.73$_{\pm0.19}$ & 131.90$_{\pm6.50}$ & 31.13$_{\pm0.74}$ & 113.75$_{\pm3.17}$ & 29.10$_{\pm0.15}$ & 28.24$_{\pm0.26}$ & 28.48$_{\pm0.25}$ & 28.86$_{\pm0.24}$ & 41.74$_{\pm5.58}$ & 29.83$_{\pm0.15}$ & 37.96$_{\pm5.41}$ & 78.80$_{\pm12.42}$ & 29.10$_{\pm0.15}$ & \textbf{26.91$_{\pm4.18}$} & 33.45$_{\pm0.96}$ & 29.27$_{\pm0.27}$ & 31.45$_{\pm0.09}$ & \underline{27.68$_{\pm0.13}$} \\
 &  & 12 & 76.41$_{\pm11.20}$ & 38.49$_{\pm0.32}$ & 132.76$_{\pm6.38}$ & 36.74$_{\pm1.27}$ & 120.15$_{\pm2.82}$ & 35.53$_{\pm0.25}$ & 34.05$_{\pm0.44}$ & 34.47$_{\pm0.23}$ & 35.11$_{\pm0.38}$ & 46.47$_{\pm4.86}$ & 36.12$_{\pm0.26}$ & 44.86$_{\pm5.89}$ & 87.00$_{\pm10.06}$ & 35.53$_{\pm0.25}$ & \textbf{31.66$_{\pm4.80}$} & 38.62$_{\pm1.73}$ & 35.68$_{\pm0.23}$ & 39.91$_{\pm0.11}$ & \underline{33.95$_{\pm0.17}$} \\
 &  & Avg & 72.73$_{\pm11.53}$ & 31.34$_{\pm0.23}$ & 132.06$_{\pm6.48}$ & 31.71$_{\pm0.83}$ & 114.33$_{\pm3.13}$ & 29.55$_{\pm0.17}$ & 28.60$_{\pm0.25}$ & 28.83$_{\pm0.25}$ & 29.25$_{\pm0.29}$ & 42.11$_{\pm5.54}$ & 30.22$_{\pm0.18}$ & 38.61$_{\pm5.26}$ & 79.96$_{\pm11.58}$ & 29.55$_{\pm0.17}$ & \textbf{27.48$_{\pm4.26}$} & 33.87$_{\pm1.02}$ & 29.75$_{\pm0.29}$ & 32.15$_{\pm0.11}$ & \underline{28.04$_{\pm0.16}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{MAPE (\%)} & 3 & 248.33$_{\pm60.12}$ & 21.84$_{\pm0.57}$ & 51.33$_{\pm3.72}$ & 23.62$_{\pm1.26}$ & 74.74$_{\pm13.07}$ & 22.70$_{\pm0.44}$ & 21.91$_{\pm0.66}$ & \underline{21.21$_{\pm0.47}$} & 23.02$_{\pm0.43}$ & 32.36$_{\pm6.82}$ & 25.09$_{\pm1.19}$ & 39.73$_{\pm11.18}$ & 72.95$_{\pm11.31}$ & 22.70$_{\pm0.44}$ & 27.97$_{\pm2.98}$ & 36.52$_{\pm2.45}$ & 23.88$_{\pm0.84}$ & 21.85$_{\pm0.34}$ & \textbf{20.48$_{\pm0.32}$} \\
 &  & 6 & 249.14$_{\pm60.20}$ & 23.93$_{\pm0.56}$ & 51.81$_{\pm3.74}$ & 24.86$_{\pm1.32}$ & 77.69$_{\pm14.94}$ & 24.38$_{\pm0.48}$ & 23.34$_{\pm0.70}$ & \underline{22.79$_{\pm0.57}$} & 24.55$_{\pm0.55}$ & 33.87$_{\pm6.63}$ & 26.49$_{\pm0.93}$ & 41.50$_{\pm9.90}$ & 74.59$_{\pm11.17}$ & 24.38$_{\pm0.48}$ & 29.14$_{\pm2.87}$ & 38.85$_{\pm2.76}$ & 25.44$_{\pm0.82}$ & 24.04$_{\pm0.25}$ & \textbf{21.87$_{\pm0.27}$} \\
 &  & 12 & 251.63$_{\pm59.90}$ & 28.83$_{\pm0.58}$ & 53.62$_{\pm3.61}$ & 28.27$_{\pm1.39}$ & 84.80$_{\pm19.50}$ & 28.22$_{\pm0.66}$ & 26.72$_{\pm0.85}$ & \underline{26.37$_{\pm0.65}$} & 28.36$_{\pm1.30}$ & 37.44$_{\pm6.32}$ & 30.18$_{\pm0.72}$ & 46.71$_{\pm9.12}$ & 81.27$_{\pm15.31}$ & 28.22$_{\pm0.66}$ & 33.05$_{\pm2.63}$ & 43.64$_{\pm3.27}$ & 28.98$_{\pm0.87}$ & 29.63$_{\pm0.52}$ & \textbf{24.65$_{\pm0.16}$} \\
 &  & Avg & 249.45$_{\pm60.06}$ & 24.44$_{\pm0.55}$ & 52.09$_{\pm3.69}$ & 25.29$_{\pm1.31}$ & 78.58$_{\pm15.42}$ & 24.78$_{\pm0.50}$ & 23.70$_{\pm0.70}$ & \underline{23.16$_{\pm0.55}$} & 25.02$_{\pm0.69}$ & 34.25$_{\pm6.60}$ & 26.96$_{\pm0.97}$ & 42.20$_{\pm9.95}$ & 75.82$_{\pm11.88}$ & 24.78$_{\pm0.50}$ & 29.72$_{\pm2.79}$ & 39.27$_{\pm2.73}$ & 25.80$_{\pm0.84}$ & 24.72$_{\pm0.32}$ & \textbf{22.09$_{\pm0.26}$} \\
\midrule
\multirow{12}{*}{\textbf{PEMS12}} & \multirow{4}{*}{MAE} & 3 & 30.52$_{\pm9.36}$ & 13.11$_{\pm0.11}$ & 30.59$_{\pm4.06}$ & 13.64$_{\pm0.09}$ & 14.82$_{\pm0.22}$ & 12.54$_{\pm0.13}$ & 12.24$_{\pm0.06}$ & 12.26$_{\pm0.06}$ & 12.24$_{\pm0.08}$ & 13.81$_{\pm1.37}$ & \underline{12.21$_{\pm0.17}$} & 12.88$_{\pm0.23}$ & 32.48$_{\pm7.23}$ & 12.54$_{\pm0.13}$ & 13.43$_{\pm0.37}$ & 15.21$_{\pm0.30}$ & 12.71$_{\pm0.27}$ & 13.12$_{\pm0.08}$ & \textbf{11.66$_{\pm0.13}$} \\
 &  & 6 & 30.89$_{\pm9.30}$ & 14.35$_{\pm0.08}$ & 31.05$_{\pm4.06}$ & 14.47$_{\pm0.11}$ & 15.79$_{\pm0.22}$ & 13.55$_{\pm0.12}$ & \underline{13.14$_{\pm0.07}$} & 13.31$_{\pm0.05}$ & 13.29$_{\pm0.09}$ & 14.74$_{\pm1.28}$ & 13.23$_{\pm0.17}$ & 13.65$_{\pm0.23}$ & 33.02$_{\pm6.56}$ & 13.55$_{\pm0.12}$ & 14.19$_{\pm0.28}$ & 16.20$_{\pm0.34}$ & 13.74$_{\pm0.23}$ & 14.49$_{\pm0.06}$ & \textbf{12.77$_{\pm0.12}$} \\
 &  & 12 & 32.40$_{\pm9.15}$ & 17.13$_{\pm0.06}$ & 32.56$_{\pm4.02}$ & 16.49$_{\pm0.19}$ & 17.68$_{\pm0.20}$ & 15.64$_{\pm0.14}$ & \textbf{14.82$_{\pm0.12}$} & 15.31$_{\pm0.06}$ & 15.30$_{\pm0.16}$ & 16.64$_{\pm1.14}$ & 15.19$_{\pm0.15}$ & 15.29$_{\pm0.37}$ & 35.00$_{\pm5.84}$ & 15.64$_{\pm0.14}$ & 16.29$_{\pm0.25}$ & 18.64$_{\pm0.63}$ & 15.94$_{\pm0.22}$ & 17.49$_{\pm0.10}$ & \underline{14.90$_{\pm0.14}$} \\
 &  & Avg & 31.14$_{\pm9.29}$ & 14.62$_{\pm0.08}$ & 31.28$_{\pm4.05}$ & 14.69$_{\pm0.10}$ & 15.93$_{\pm0.21}$ & 13.72$_{\pm0.13}$ & \underline{13.24$_{\pm0.07}$} & 13.44$_{\pm0.05}$ & 13.42$_{\pm0.09}$ & 14.89$_{\pm1.28}$ & 13.36$_{\pm0.17}$ & 13.79$_{\pm0.25}$ & 33.29$_{\pm6.42}$ & 13.72$_{\pm0.13}$ & 14.45$_{\pm0.30}$ & 16.49$_{\pm0.36}$ & 13.94$_{\pm0.24}$ & 14.77$_{\pm0.07}$ & \textbf{12.92$_{\pm0.13}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{RMSE} & 3 & 45.00$_{\pm12.05}$ & 22.80$_{\pm0.20}$ & 55.46$_{\pm7.36}$ & 23.14$_{\pm0.27}$ & 23.98$_{\pm0.17}$ & 21.62$_{\pm0.14}$ & 21.31$_{\pm0.10}$ & \underline{21.25$_{\pm0.09}$} & 21.32$_{\pm0.06}$ & 23.70$_{\pm3.00}$ & 21.32$_{\pm0.21}$ & 21.96$_{\pm0.26}$ & 47.90$_{\pm9.87}$ & 21.62$_{\pm0.14}$ & 23.23$_{\pm0.50}$ & 25.07$_{\pm0.38}$ & 21.90$_{\pm0.25}$ & 22.93$_{\pm0.06}$ & \textbf{20.67$_{\pm0.14}$} \\
 &  & 6 & 45.98$_{\pm11.88}$ & 25.43$_{\pm0.15}$ & 56.48$_{\pm7.36}$ & 24.92$_{\pm0.27}$ & 26.05$_{\pm0.19}$ & 23.80$_{\pm0.15}$ & \underline{23.19$_{\pm0.12}$} & 23.43$_{\pm0.08}$ & 23.55$_{\pm0.11}$ & 25.65$_{\pm2.73}$ & 23.47$_{\pm0.19}$ & 23.67$_{\pm0.26}$ & 49.64$_{\pm9.15}$ & 23.80$_{\pm0.15}$ & 24.79$_{\pm0.36}$ & 26.94$_{\pm0.28}$ & 24.04$_{\pm0.21}$ & 25.89$_{\pm0.04}$ & \textbf{22.94$_{\pm0.13}$} \\
 &  & 12 & 48.98$_{\pm11.57}$ & 30.74$_{\pm0.15}$ & 59.28$_{\pm7.23}$ & 28.72$_{\pm0.33}$ & 29.75$_{\pm0.26}$ & 27.83$_{\pm0.22}$ & \textbf{26.41$_{\pm0.21}$} & 27.27$_{\pm0.10}$ & 27.47$_{\pm0.27}$ & 29.31$_{\pm2.35}$ & 27.21$_{\pm0.17}$ & \underline{26.75$_{\pm0.56}$} & 53.94$_{\pm8.91}$ & 27.83$_{\pm0.22}$ & 28.54$_{\pm0.37}$ & 31.31$_{\pm0.71}$ & 28.21$_{\pm0.23}$ & 31.74$_{\pm0.07}$ & 26.94$_{\pm0.18}$ \\
 &  & Avg & 46.38$_{\pm11.85}$ & 25.84$_{\pm0.17}$ & 56.84$_{\pm7.33}$ & 25.25$_{\pm0.26}$ & 26.24$_{\pm0.19}$ & 24.04$_{\pm0.16}$ & \underline{23.32$_{\pm0.13}$} & 23.62$_{\pm0.08}$ & 23.74$_{\pm0.13}$ & 25.87$_{\pm2.73}$ & 23.64$_{\pm0.19}$ & 23.83$_{\pm0.30}$ & 50.01$_{\pm9.12}$ & 24.04$_{\pm0.16}$ & 25.17$_{\pm0.41}$ & 27.41$_{\pm0.30}$ & 24.33$_{\pm0.23}$ & 26.33$_{\pm0.04}$ & \textbf{23.13$_{\pm0.14}$} \\
\cmidrule(lr){2-22}
 & \multirow{4}{*}{MAPE (\%)} & 3 & 189.12$_{\pm81.54}$ & 24.22$_{\pm0.89}$ & 35.89$_{\pm2.38}$ & 24.80$_{\pm0.77}$ & 27.93$_{\pm0.88}$ & 25.12$_{\pm1.29}$ & 23.97$_{\pm0.53}$ & \underline{22.82$_{\pm0.48}$} & 23.83$_{\pm0.63}$ & 27.15$_{\pm2.01}$ & 24.21$_{\pm1.48}$ & 28.87$_{\pm3.67}$ & 98.94$_{\pm55.89}$ & 25.12$_{\pm1.29}$ & 29.91$_{\pm1.34}$ & 49.43$_{\pm6.57}$ & 26.55$_{\pm1.53}$ & 23.91$_{\pm0.76}$ & \textbf{22.15$_{\pm0.24}$} \\
 &  & 6 & 189.83$_{\pm81.85}$ & 26.25$_{\pm0.99}$ & 36.06$_{\pm2.60}$ & 26.07$_{\pm0.94}$ & 28.97$_{\pm1.05}$ & 26.28$_{\pm1.11}$ & 24.98$_{\pm0.53}$ & \underline{23.96$_{\pm0.33}$} & 24.78$_{\pm0.57}$ & 28.11$_{\pm1.60}$ & 25.43$_{\pm1.18}$ & 29.43$_{\pm3.01}$ & 100.19$_{\pm57.31}$ & 26.28$_{\pm1.11}$ & 31.55$_{\pm1.74}$ & 52.52$_{\pm7.86}$ & 27.55$_{\pm1.47}$ & 26.21$_{\pm0.77}$ & \textbf{23.50$_{\pm0.20}$} \\
 &  & 12 & 192.38$_{\pm81.45}$ & 31.60$_{\pm1.38}$ & 39.47$_{\pm2.90}$ & 29.76$_{\pm1.38}$ & 31.53$_{\pm1.19}$ & 29.32$_{\pm0.88}$ & 27.65$_{\pm0.60}$ & \underline{27.15$_{\pm0.39}$} & 27.91$_{\pm0.65}$ & 30.63$_{\pm1.05}$ & 28.60$_{\pm0.78}$ & 31.89$_{\pm3.03}$ & 103.43$_{\pm58.72}$ & 29.32$_{\pm0.88}$ & 36.84$_{\pm2.23}$ & 60.18$_{\pm10.87}$ & 30.38$_{\pm1.29}$ & 32.33$_{\pm1.08}$ & \textbf{26.16$_{\pm0.25}$} \\
 &  & Avg & 190.26$_{\pm81.74}$ & 26.91$_{\pm1.03}$ & 36.87$_{\pm2.61}$ & 26.58$_{\pm1.00}$ & 29.25$_{\pm0.95}$ & 26.64$_{\pm1.12}$ & 25.29$_{\pm0.55}$ & \underline{24.35$_{\pm0.38}$} & 25.20$_{\pm0.58}$ & 28.38$_{\pm1.60}$ & 25.81$_{\pm1.11}$ & 29.83$_{\pm3.17}$ & 100.49$_{\pm57.31}$ & 26.64$_{\pm1.12}$ & 32.31$_{\pm1.73}$ & 53.41$_{\pm8.13}$ & 27.94$_{\pm1.43}$ & 26.98$_{\pm0.82}$ & \textbf{23.70$_{\pm0.21}$} \\
\bottomrule
\end{tabular}%
}
\end{table*}

